A Convergence Analysis of Approximate Message Passing with Non-Separable Functions and Applications to Multi-Class Classification

Motivated by the recent application of approximate message passing (AMP) to the analysis of convex optimizations in multi-class classifications [Loureiro, et. al., 2021], we present a convergence analysis of AMP dynamics with non-separable multivariate nonlinearities. As an application, we present a complete (and independent) analysis of the motivated convex optimization problem.

==> trash.tex <==
\author{%
  \IEEEauthorblockN{Burak \c{C}akmak}
  \IEEEauthorblockA{Technical University of  Berlin\\Berlin, Germany\\ Email: burak.cakmak@tu-berlin.de}
  \and
\IEEEauthorblockN{Yue M. Lu}
  \IEEEauthorblockA{Harvard University,  \\ Cambridge, MA 02138, USA\\ Email: yuelu@seas.harvard.edu}
  \and
  \IEEEauthorblockN{Manfred Opper}
  \IEEEauthorblockA{Technical University of  Berlin\\Berlin, Germany\\ Email: manfred.opper@tu-berlin.de}
}
